Generalized Paxos Made Byzantine (and Less Complex)

One of the most recent members of the Paxos family of protocols is Generalized Paxos. This variant of Paxos has the characteristic that it departs from the original specification of consensus, allowing for a weaker safety condition where different processes can have a different views on a sequence being agreed upon. However, much like the original Paxos counterpart, Generalized Paxos does not have a simple implementation. Furthermore, with the recent practical adoption of Byzantine fault tolerant protocols, it is timely and important to understand how Generalized Paxos can be implemented in the Byzantine model. In this paper, we make two main contributions. First, we provide a description of Generalized Paxos that is easier to understand, based on a simpler specification and the pseudocode for a solution that can be readily implemented. Second, we extend the protocol to the Byzantine fault model.

==> algo_bft.tex <==
\iffalse\section{Byzantine Generalized Paxos Pseudocode} \label{bft_code}
This section presents the pseudocode for the Byzantine Generalized Paxos protocol. \par
\noindent \textbf{Checkpointing} The pseudocode includes a checkpointing feature that allows the leader to propose a special command $C^*$ that causes both the acceptors and learners to discard previously stored commands. This feature can be used to prevent commands from being stored indefinitely. However, since commands are kept at the acceptors to ensure that they will eventually be committed, special care has to be taken before discarding them. To prevent unlearned commands from being discarded, the checkpointing command must be sent within a sequence in a classic ballot. In phase 1 of that classic ballot, acceptors send every command they have to the leader, who waits for $N-f$ phase 1b messages. The leader can be sure that the commands were originated from proposers by verifying the signatures they contain. Since, when proposing to acceptors in fast ballots, proposers wait for acknowledgments from $N-f$ proposers, there's at least one correct acceptor in the intersection of a quorum that received a proposal and a quorum that sends commands to the leader. This means that any proposed value will be sent by some acceptor to the leader and included in the leader's sequence, along with the checkpointing command. Since acceptors must be certain that it's safe to discard previously stored commands, before sending phase 2b messages to learners, they first broadcast these messages among themselves. This round between acceptors is necessary because a Byzantine leader could send a checkpointing command to some acceptors but not others. After waiting for $N-f$ such messages, acceptors send phase 2b messages to the learners along with the cryptographic proofs exchanged in the acceptor-to-acceptor broadcast. After receiving just one message, the leader may simply validate the $N-f$ acceptor proofs contained in it and learn the commands. The learners discard previously stored state when they execute the checkpointing command.
\fi





==> algo_cft.tex <==
\begin{table}[h!]
	\renewcommand{\arraystretch}{1.5}
	\centering
	\begin{tabular}{ |c|c|}
		\hline
		\multicolumn{2}{|c|}{Notation}\\
		\hline
		Symbol & Definition \\
		\hline
		$\sqcup$ & least upper bound \\
		\hline
		$\sqcap$ & greatest lower bound \\
		\hline
		$\bullet$ & append operator \\
		\hline
	\end{tabular} 
	\caption{Notation for the pseudocode} 
	\label{table:1}
\end{table}

\begin{algorithm}
	\caption{Generalized Paxos - Proposer p}
	\begin{algorithmic}[1]
		
		\Function{propose}{\textit{C}}
		\If{fast\_ballot}
		\State \Call{send}{$fast, C$} to Acceptors;
		\Else
		\State \Call{send}{\textit{propose, C}} to Leader;
		\EndIf
		\EndFunction
		
		
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{Generalized Paxos - Leader l}
	\textbf{Local variables:} $ballot_l = 0,\ maxTried_l = \bot,\ C_l = \bot, messages = \bot$
	\begin{algorithmic}[1]
		\State \textbf{upon} \textit{receive(propose, C)} from proposer $p_i$ \textbf{do} 
		\State \hspace{\algorithmicindent} $C_l = C$;
		\State \hspace{\algorithmicindent} \Call{phase\_1a}{$ $};
		\State
		\State \textbf{upon} \textit{receive(statement)} from acceptor $a_i$ \textbf{do}
		\State \hspace{\algorithmicindent}  $messages[ballot_l][a_i] = statement$;
		\State \hspace{\algorithmicindent} \textbf{if} $\#(messages) \geq \lfloor \frac{N}{2} \rfloor +1$ \textbf{then} 
		\State \hspace{\algorithmicindent}\hspace{\algorithmicindent} \Call{phase\_2a}{$ballot_l, Q$};
		\State
		%\item[] % unnumbered empty line
		\Function{phase\_1a}{}
		\State \Call{send}{$p1a, ballot_l$} to Acceptors;
		\EndFunction
		
		\State
		\Function{phase\_2a}{$bal, Q$}
		\State $maxTried_l$ = \Call{proved\_safe}{$Q, bal$};
		\State $maxTried_l = maxTried_l \bullet C_l$;
		\State \Call{send}{$p2a,ballot_l, maxTried_l$} to Acceptors;
		\EndFunction
		
		\State
		\Function{proved\_safe}{$ballot$}
		\State $maxTried = \bot$;
		\State \textbf{for} $val$ in $message[ballot]$ \textbf{do}
		\State \hspace{\algorithmicindent} \textbf{if} $maxTried = \bot$ or $\Call{is\_prefix}{val, maxTried}$ \textbf{then}
		\State\hspace{\algorithmicindent}\hspace{\algorithmicindent} $maxTried = val$;
		\State \textbf{end for}
		\State \textbf{return} $maxTried$;
		\EndFunction
		
			\State
		\Function{is\_prefix}{$new\_sequence, old\_sequence$}
		\If {$\lVert old\_sequence \rVert > \lVert new\_sequence \rVert$}
		\State \textbf{return} \textit{false};
		\EndIf
		
		\State
		\item[] outer:	
		\State \textbf{for} $c_{old}$ in $old\_sequence$ \textbf{do}
		\State \hspace{\algorithmicindent} \textbf{for} $c_{new}$ in $new\_sequence$ \textbf{do}
		\State\hspace{\algorithmicindent}\hspace{\algorithmicindent} \textbf{if} $c_{old} = c_{new}$ \textbf{then}
		\State \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} \textbf{continue} \textit{outer};
		
		\State \hspace{\algorithmicindent}\hspace{\algorithmicindent} \textbf{else if} !\Call{are\_commutative}{$c_{old}, c_{new}$} \textbf{then}
		\State\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} \textbf{return} \textit{false};
		\State \hspace{\algorithmicindent}\textbf{end for}
		\State \hspace{\algorithmicindent}\textbf{return} \textit{false};
		\State \textbf{end for}
		\State
		\State \textbf{return} \textit{true};
		\EndFunction
		
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{Generalized Paxos - Acceptor a}
	\textbf{Local variables: } $bal_a = 0,\ val_a = \bot$ 
	\begin{algorithmic}[1]
		
		\State \textbf{upon} \textit{receive(fast, val)} from proposer \textit{p} \textbf{do}
		\State \hspace{\algorithmicindent} \Call{phase\_2b\_fast}{$val$};
		
		\State
		\State \textbf{upon} \textit{receive(p1a, ballot)} from leader \textit{l} \textbf{do}
		\State \hspace{\algorithmicindent} \Call{phase\_1b}{$ballot, l$};
		
		\State
		\State \textbf{upon} \textit{receive(p2a, ballot, value)} from leader \textit{l} \textbf{do}
		\State \hspace{\algorithmicindent} \Call{phase\_2b\_classic}{$ballot, value$};
		
		\State
		\Function{phase\_1b}{$m, l$}
		\If {$bal_a < m$}
		\State \Call{send}{$p1b, m, bal_a, val_a$} to leader l;
		\State $bal_a = m$;
		\EndIf
		\EndFunction
		
		\State
		\Function{phase\_2b\_classic}{$m, v$}
		\State $k = max(i\ |\ (i < m) \wedge (\exists a \in Q :\ val_a[i]\ \neq null))$;
		\If {$m \geq k$}
		\State $val_a = v$;
		\State \Call{send}{$p2b, bal_a, val_a$} to learners;
		\EndIf
		\EndFunction
		
		\State
		\Function{phase\_2b\_fast}{$v$}
		\State $k = max(i\ |\ (i < m) \wedge (\exists a \in Q :\ val_a[i]\ \neq null))$;
		\If {$bal_a == k$}
		\State $val_a = val_a \bullet v$;
		\State \Call{send}{$p2b, bal_a, val_a$} to learners;
		\EndIf
		\EndFunction
		
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{Generalized Paxos - Learner l}
	\textbf{Local variables: } $learned = \bot, messages = \bot$ 
	\begin{algorithmic}[1]
		\State \textbf{upon} \textit{receive($p2b, bal, val$)} from acceptor $a_i$ \textbf{do}
		\State \hspace{\algorithmicindent} $messages[bal][a_i] = val$;
		\State \hspace{\algorithmicindent} \textbf{if} {($fast\_ballot$ and $\#(messages[bal]) \geq \lceil \frac{3N}{4} \rceil$) or
			\State \hspace{\algorithmicindent} \hspace{\algorithmicindent}	($classic\_ballot$ and $\#(messages[bal]) \geq \lfloor \frac{N}{2}\rfloor+1$)} \textbf{then}
		\State \hspace{\algorithmicindent} \hspace{\algorithmicindent} \hspace{\algorithmicindent} $learned = learned \sqcup val$;
	\end{algorithmic}
\end{algorithm}


==> cft_desc.tex <==
\textbf{Simplified Problem} Generalized Paxos solves the problem of agreeing on increasing sets of values. These sets of commands are defined to be \textit{c-structs}, which are structures more generic than sequences since they allow for command sequences $\sigma$ and $\tau$ to be equivalent despite having different contents. This is possible because there is a custom \textit{equivalence relation} between \textit{c-structs}. However, this generalization comes at the cost of increased complexity. To present a simpler version of the protocol, our simplification does away with the generic equivalence relation and defines it to be as the equivalence relation between command histories.  \par
\textbf{Protocol} \textcolor{red}{Finish CFT protocol description}

==> prelims.tex <==


